OpenTSLM TeeMoE: A Unified Time-Series Language Model for Forecasting, Contextual Prediction, and Reasoning

Real-world time-series applications increasingly require models that can handle time series forecasting, context-conditioned prediction, and language-based temporal reasoning. Yet current time-series foundation models remain fragmented across these capabilities: numerical specialists often provide the strongest forecasts, while language-based models offer broader contextual understanding and analysis. A central challenge is to unify these heterogeneous capabilities without reducing their individual performance. We introduce OpenTSLM TeeMoE, a generalist time-series language model that can forecast directly from observed time series, reason over textual context and temporal patterns, and synthesize and refine predictions from external numerical forecasting specialists. We independently train three low-rank experts for forecast aggregation, native forecasting, and temporal analysis over a shared backbone. A learned LoRA mixture-of-experts controller then weights their frozen parameter updates for each request. Our proposed model achieves strong performance on widely used benchmarks for time series forecasting, context-conditioned prediction, and language-based temporal reasoning, ranking among the top three on GIFT-Eval by mean MASE rank, Context is Key by RCRPS, and TimeSeriesExam by accuracy.

==> appendices/recipe_format.tex <==
\RequirePackage{framed}
\RequirePackage{needspace}
\newenvironment{recipebox}[1]{\par\addvspace{1em}\Needspace{7\baselineskip}
  \long\def\MidFrameCommand##1{\fboxrule=\FrameRule\fboxsep=\FrameSep
    \fbox{\vbox{\hbox{\strut\textbf{#1 (continued)}}\smallskip\hbox{##1}}}}\let\LastFrameCommand\MidFrameCommand
  \begin{framed}\textbf{#1}\par\smallskip
}{\end{framed}\par
}
\newcommand{\recipedivider}{\par\medskip\hrule\medskip
  \noindent\textbf{Training data}\par\smallskip
}
\newcommand{\recipedatarow}[2]{\textbullet\enspace #1 & #2\\}
\newenvironment{recipedatalist}{\begin{list}{\textbullet}{\setlength{\leftmargin}{1.2em}\setlength{\labelwidth}{0.7em}\setlength{\labelsep}{0.5em}\setlength{\itemsep}{1pt}\setlength{\parsep}{0pt}\setlength{\topsep}{2pt}}}{\end{list}}
\newcommand{\recipedataitem}[2]{\item #1\hfill\mbox{#2}}

